Machine Translation Evaluation Meets Community Question Answering

We explore the applicability of machine translation evaluation (MTE) methods to a very different problem: answer ranking in community Question Answering. In particular, we adopt a pairwise neural network (NN) architecture, which incorporates MTE features, as well as rich syntactic and semantic embeddings, and which efficiently models complex non-linear interactions. The evaluation results show state-of-the-art performance, with sizeable contribution from both the MTE features and from the pairwise NN architecture.

==> introduction-paco.tex <==
%%%
%%% Section 1: Introduction
%%%


In our community Question Answering (cQA) task, we are given a question from a community forum and a thread of associated text comments intended to answer the given question; and the goal is to rank the comments according to their appropriateness to the question. Since cQA forum threads are noisy, as many comments are not answers to the question, the challenge lies in learning to rank all \emph{good} comments above all \emph{bad} comments.\footnote{In practice, we adopt the definition of the task and the datasets from SemEval--2016 Task 3 on ``Community Question Answering''. See the task website for details and examples (http://alt.qcri.org/semeval2016/task3/)} %See the upcoming task description paper for details~\cite{nakov-EtAl:2016:SemEval}.
 In this paper, we tackle the task from a novel perspective: by using notions of %explore a novel approach to the application of a 
 machine translation evaluation (MTE) %system to a seemingly very different problem, that is, %\emph{question--comment similarity} 
%answer ranking in community Question Answering (cQA). 
to decide on the \emph{quality} of a comment. 

From a general viewpoint, the two tasks seem similar: both are reasoning about the similarity of two competing texts against a reference text, to decide which one is better. In MTE, the goal is to decide whether a hypothesis translation conveys the same meaning as the reference translation. In cQA, it is to determine whether the comment is an appropriate answer to the question. However, there are some profound differences which have implications on how each task is solved. In MTE, we can expect shorter texts, which are much more similar among them. In cQA, the question and the intended answers might differ significantly both in length and in lexical content. Thus, it is not clear a priori whether the MTE network can work well to address the cQA problem. Here, we show that the analogy is not only convenient, but it can achieve state-of-the-art results.

In particular, we extend the pairwise neural network framework from~\newcite{guzman-EtAl:2015:ACL-IJCNLP} to suit our purpose. %In that work, MTE is approached in a pairwise fashion, i.e., given two translation hypotheses and a reference translation to compare to, the task is to decide which translation hypothesis is better.
%We are aware of neural network (NN) models applied to cQA tasks: question-question similarity \cite{zhou-EtAl:2015,dossantos-EtAl:2015,LeiJBJTMM15}
%and answer selection \cite{severyn2015sigir,wang-nyberg:2015:ACL-IJCNLP,shen2015word,feng2015applying,tan2015lstm}.
%However, here the goal is different, we adapt an existing NN from a different but related problem.
%
%There is also work that uses machine translation model(s) as a feature(s)
%\cite{Berger:2000:BLC:345508.345576,Echihabi:2003:NAQ:1075096.1075099,jeon2005finding,Soricut:2006:AQA:1127331.1127342,riezler-EtAl:2007:ACLMain,li2011improving,Surdeanu:2011:LRA:2000517.2000520},
%e.g., a variation of IBM model 1, to compute the probability that the question is a ``translation'' of the candidate answer.
%Unlike that work, here we port an entire MTE framework to the cQA problem.
%
We believe that the MTE neural network architecture %from~\newcite{guzman-EtAl:2015:ACL-IJCNLP} 
is interesting for this problem because: \Ni it works by comparing pairs of competing comments, which is appropriated for a ranking problem; \Nii it allows for an easy incorporation of rich syntactic and semantic embedded representations of the input texts, and it efficiently models complex non-linear relationships among them; \Niii it uses a number of MT evaluation measures that have not been used for the cQA task (e.g., TER, Meteor, BLEU).

To validate our intuitions, we present series of experiments using the publicly available SemEval-2016 Task 3 datasets. 
%\footnote{http://alt.qcri.org/semeval2016/task3/} 
%with remarkably good results. 
We show that a naive application of the MTE architecture and features on the cQA task already yields results that are largely above the task baselines. Furthermore, by adapting the models %retrain the word embeddings 
with in-domain data, and adding lightweight task-specific features; %described in the related literature, 
we are able to boost our system to reach state-of-the-art performance. %(i.e., second-best result compared to the SemEval-2016 Task 3 systems). 
More interestingly, we analyze the contribution of several features and parts of the NN architecture by performing an ablation study. We observe that every single piece contributes important information to achieve the final performance. While task-specific features are crucial, other aspects of the framework are relevant as well: syntactic embeddings, MT evaluation measures, and pairwise training of the network.

\paragraph{Related Work} Recently, many neural network (NN) models have been applied to cQA tasks: e.g.,  \emph{question-question similarity} \cite{zhou-EtAl:2015,dossantos-EtAl:2015,LeiJBJTMM15}
and \emph{answer selection} \cite{severyn2015sigir,wang-nyberg:2015:ACL-IJCNLP,shen2015word,feng2015applying,tan2015lstm}.
However, here the goal is different, we adapt an existing NN from a different but related problem.
%
There is also work that uses machine translation model(s) as a feature(s)
\cite{Berger:2000:BLC:345508.345576,Echihabi:2003:NAQ:1075096.1075099,jeon2005finding,Soricut:2006:AQA:1127331.1127342,riezler-EtAl:2007:ACLMain,li2011improving,Surdeanu:2011:LRA:2000517.2000520},
e.g., a variation of IBM model 1, to compute the probability that the question is a ``translation'' of the candidate answer.
Unlike that work, here we port an entire MTE framework to the cQA problem.



==> introduction.bak.tex <==
%%%
%%% Section 1: Introduction
%%%

We explore the application of a machine translation evaluation (MTE) system to a seemingly very different problem, that is, %\emph{question--comment similarity} 
answer ranking in community Question Answering (cQA). In particular, we chose the neural network from~\newcite{guzman-EtAl:2015:ACL-IJCNLP}. In that work, MTE is approached in a pairwise fashion, i.e., given two translation hypotheses and a reference translation to compare to, the task is to decide which translation hypothesis is better.

In the cQA task, we assume to be given a question from a community forum and a thread of associated text comments intended to answer the given question. Since cQA forums are very noisy, many of the comments are not really good answers. The goal here is to rank the comments according to their appropriateness to the question, placing all \emph{good} comments above all \emph{bad} comments. In practice, we adopt the definition of the task and the datasets from SemEval--2016 Task 3 on ``Community Question Answering''. See the task website for details and examples (http://alt.qcri.org/semeval2016/task3/). %See the upcoming task description paper for details~\cite{nakov-EtAl:2016:SemEval}.
 
%We are aware of neural network (NN) models applied to cQA tasks: question-question similarity \cite{zhou-EtAl:2015,dossantos-EtAl:2015,LeiJBJTMM15}
%and answer selection \cite{severyn2015sigir,wang-nyberg:2015:ACL-IJCNLP,shen2015word,feng2015applying,tan2015lstm}.
%However, here the goal is different, we adapt an existing NN from a different but related problem.
%
%There is also work that uses machine translation model(s) as a feature(s)
%\cite{Berger:2000:BLC:345508.345576,Echihabi:2003:NAQ:1075096.1075099,jeon2005finding,Soricut:2006:AQA:1127331.1127342,riezler-EtAl:2007:ACLMain,li2011improving,Surdeanu:2011:LRA:2000517.2000520},
%e.g., a variation of IBM model 1, to compute the probability that the question is a ``translation'' of the candidate answer.
%Unlike that work, here we port an entire MTE framework to the cQA problem.

The analogy we apply to adapt the MTE architecture to the cQA problem is the following: given two comments $c_1$ and $c_2$ from the question thread (which play the role of the two competing translation hypotheses), we have to decide whether $c_1$ is a better answer than $c_2$ to question $q$ (which plays the role of the translation reference). If we assume the existence of such a function $f(q,c_1,c_2)$, we can rank the finite list of comments in the thread by comparing all possible pairs and by accumulating for each comment the scores given by $f$.

We believe that the MTE neural network architecture from~\newcite{guzman-EtAl:2015:ACL-IJCNLP} is interesting for this problem because: \Ni it works by comparing pairs of competing comments, which might be good for a ranking problem; \Nii it allows for an easy incorporation of rich syntactic and semantic embedded representations of the input texts, and it efficiently models complex non-linear relationships among them; \Niii it uses a number of MT evaluation measures that have not been used for the cQA task (e.g., TER, Meteor, BLEU).

Note that, from a general viewpoint, the two tasks are similar: both are reasoning about the similarity of two competing texts against a reference text, to decide which one is better. However, the semantic task to be solved is quite different. In MTE, the goal is to decide whether a hypothesis translation conveys the same meaning as the reference translation. In cQA, it is to determine whether the comment is an appropriate answer to the question. In MTE, we can expect shorter texts, which are much more similar among them. In cQA, the question and the intended answers might differ significantly both in length and in lexical content. Thus, it is not clear a priori whether the MTE network can work well for the cQA problem.

We present series of experiments using the publicly available SemEval-2016 Task 3 datasets
%\footnote{http://alt.qcri.org/semeval2016/task3/} 
with remarkably good results. By just reproducing the MTE architecture and features on the cQA dataset, we already obtain results that are largely above the task baselines. If we just retrain the word embeddings with in-domain data and we add some lightweight task-specific features, described in the related literature, we are able to boost our system to reach state-of-the-art performance %(i.e., second-best result compared to the SemEval-2016 Task 3 systems). 
More interestingly, we analyze the contribution of several features and parts of the NN architecture by performing an ablation study. We can see that every single piece contributes important information to achieve the final performance. Of course, the task-specific features are very important, but the following are relevant aspects as well: syntactic embeddings, MT evaluation measures, and pairwise training of the network.

\paragraph{Related Work} Recently, many neural network (NN) models have been applied to cQA tasks: e.g.,  \emph{question-question similarity} \cite{zhou-EtAl:2015,dossantos-EtAl:2015,LeiJBJTMM15}
and \emph{answer selection} \cite{severyn2015sigir,wang-nyberg:2015:ACL-IJCNLP,shen2015word,feng2015applying,tan2015lstm}.
However, here the goal is different, we adapt an existing NN from a different but related problem.
%
There is also work that uses machine translation model(s) as a feature(s)
\cite{Berger:2000:BLC:345508.345576,Echihabi:2003:NAQ:1075096.1075099,jeon2005finding,Soricut:2006:AQA:1127331.1127342,riezler-EtAl:2007:ACLMain,li2011improving,Surdeanu:2011:LRA:2000517.2000520},
e.g., a variation of IBM model 1, to compute the probability that the question is a ``translation'' of the candidate answer.
Unlike that work, here we port an entire MTE framework to the cQA problem.



==> model.bak.tex <==
%%%
%%% Section 2: Neural Model for Answer Relevance Ranking
%%%

The NN model we use for answer ranking is depicted in Figure~\ref{fig:architecture}. It is a direct adaptation of the feed-forward NN for MTE described in~\cite{guzman-EtAl:2015:ACL-IJCNLP}. 
Technically, we have a binary classification task with input $(q,c_1,c_2)$, which should output 1 if $c_1$ is better answer to $q$ than $c_2$, and 0 otherwise.
%\footnote{In this work, we do not learn to predict ties, and ties are excluded from our training data.} 
The network computes a sigmoid function $f(q,c_1,c_2)=\sig(\mathbf{w^T_v}\phi(q,c_1,c_2) + b_v)$, 
where $\phi(x)$  transforms the input $x$ through the hidden layer, $\mathbf{w_v}$ are the weights from the hidden layer to the output layer, and $b_v$ is a bias term. 

\begin{figure}[t]
\centering
\hspace*{-2mm}\includegraphics[width=.5\textwidth]{imgs/architecture_color}
\caption{\label{fig:architecture} Overall architecture of the NN.}
\end{figure}

We first map the question and the comments to a fixed-length vector $\left[ \mathbf{x}_q, \mathbf{x}_{c_1},  \mathbf{x}_{c_2} \right]$, using syntactic and semantic embeddings. Then, we feed this vector as input to the neural network, which models three types of interactions, using different groups of nodes in the hidden layer. 
There are two \emph{evaluation} groups $\mathbf{h_{q1}}$ and $\mathbf{h_{q2}}$
that model how good each comment $c_i$ is to the question $q$.
The input to these groups are the concatenations $\left[ \mathbf{x}_q, \mathbf{x}_{c_1} \right]$ and $\left[\mathbf{x}_{q}, \mathbf{x}_{c_2} \right]$, respectively.
%
The third group of hidden nodes $\mathbf{h_{12}}$, which we call \emph{similarity} group, models how close $c_1$ and $c_2$ are. Its input is $\left[ \mathbf{x}_{c_1}, \mathbf{x}_{c_2} \right]$.
This might be useful as highly similar comments are likely to be comparable in appropriateness, irrespective of whether they are good or bad answers in absolute terms.
%
In summary, the transformation $\phi(q,c_1,c_2) = [\mathbf{h_{q1}}, \mathbf{h_{q2}}, \mathbf{h_{12}}]$ can be written as:
\vspace*{-0.5mm}
%
\begin{eqnarray*}
 \mathbf{h_{qi}} &=& g( \mathbf{W_{qi}} \mathbf{\left[ \mathbf{x}_q, \mathbf{x}_{c_i} \right]} + \mathbf{b_{qi}}),\, i=1,2\\
 \mathbf{h_{12}} &=& g( \mathbf{W_{12}} \mathbf{\left[ \mathbf{x}_{c_1}, \mathbf{x}_{c_2} \right]} +  \mathbf{b_{12}}),
\vspace*{-1mm}
\end{eqnarray*}
\noindent where $g(.)$ is a non-linear activation function (applied component-wise), $\mathbf{W} \in \real^{H \times N}$ are the associated weights between the input layer and the hidden layer, and $\mathbf{b}$ are the corresponding bias terms. We use $\tanh$ as an activation function, rather than $\sig$, to be consistent with how parts of our input vectors are generated.\footnote{The input word embeddings are trained with NNs that used $\tanh$ as an activation function.} 

The model further allows to incorporate external sources of information in the form of \emph{skip arcs} that go directly from the input to the output, skipping the hidden layer. These arcs represent pairwise \emph{similarity} feature vectors between $q$ and either $c_1$ or $c_2$. In these feature vectors, we encode MT evaluation measures (e.g., TER, Meteor, and BLEU), cQA task-specific features, etc. See Section~\ref{subsec:features} for detail about the features implemented as skip arcs. In the figure, we indicate these pairwise external feature sets as $\psi(q,c_1)$ and  $\psi(q,c_2)$. When including the external features, the activation at the output is:
$f(q,c_1,c_2)=\sig(\mathbf{w^T_v} [\phi(q,c_1,c_2), \psi(q,c_1), \psi(q,c_2)] + b_v)$.

%%% Network training
%We implemented the network using Theano \cite{bergstra+al:2010-scipy}. 
%We trained our network with stochastic gradient descent (SGD), to minimize the negative log likelihood of the training data for the parameters of the model. We employed a regularized cost function with $L_2$ regularization. We used mini-batches and adagrad updates~\cite{Duchi11}.


